Precoded Integer-Forcing Universally Achieves the MIMO Capacity to Within a Constant Gap

An open-loop single-user multiple-input multiple-output communication scheme is considered where a transmitter, equipped with multiple antennas, encodes the data into independent streams all taken from the same linear code. The coded streams are then linearly precoded using the encoding matrix of a perfect linear dispersion space-time code. At the receiver side, integer-forcing equalization is applied, followed by standard single-stream decoding. It is shown that this communication architecture achieves the capacity of any Gaussian multiple-input multiple-output channel up to a gap that depends only on the number of transmit antennas.

==> cube.tex <==
%\psline[linewidth=0.5pt,fillstyle=solid,linecolor=orange](-5,-5)(-5,5)(5,5)(5,-5)(-5,-5)
\psframe[linecolor=yellow,fillstyle=solid,fillcolor=yellow](-5,-5)(5,5)
\pscircle[linecolor=black,fillstyle=solid,fillcolor=orange](0,0){2}


==> hline.tex <==
\psline[linewidth=0.3pt,linecolor=black](50,0)(-40,0)
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](50,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](40,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](30,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](20,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](10,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](-40,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](-30,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](-20,0){1}
\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](-10,0){1}



==> lattice1Dq11.tex <==

\psset{unit=0.6mm}
\psline[linecolor=black,fillstyle=solid,fillcolor=black](0,-22)(0,22)

\rput(0,-20){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,-16){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,-12){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,-8){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,-4){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,0){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,4){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,8){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,12){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,16){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}
\rput(0,20){\pscircle[linecolor=black,fillstyle=solid,fillcolor=black](0,0){1}}

==> vline.tex <==
\psline[linewidth=0.3pt,linecolor=black](0,-40)(0,50)

